ProJudge: A Multi-Modal Multi-Discipline Benchmark and Instruction-Tuning Dataset for MLLM-based Process Judges

As multi-modal large language models (MLLMs) frequently exhibit errors when solving scientific problems, evaluating the validity of their reasoning processes is critical for ensuring reliability and uncovering fine-grained model weaknesses. Since human evaluation is laborious and costly, prompting MLLMs as automated process judges has become a common practice. However, the reliability of these model-based judges remains uncertain. To address this, we introduce ProJudgeBench, the first comprehensive benchmark specifically designed for evaluating abilities of MLLM-based process judges. ProJudgeBench comprises 2,400 test cases and 50,118 step-level labels, spanning four scientific disciplines with diverse difficulty levels and multi-modal content. In ProJudgeBench, each step is meticulously annotated by human experts for correctness, error type, and explanation, enabling a systematic evaluation of judges' capabilities to detect, classify and diagnose errors. Evaluation on ProJudgeBench reveals a significant performance gap between open-source and proprietary models. To bridge this gap, we further propose ProJudge-173k, a large-scale instruction-tuning dataset, and a Dynamic Dual-Phase fine-tuning strategy that encourages models to explicitly reason through problem-solving before assessing solutions. Both contributions significantly enhance the process evaluation capabilities of open-source models. All the resources will be released to foster future research of reliable multi-modal process evaluation.

==> images/bar_step_position_acc.tex <==
\begin{figure}[!t]
\centering
  \resizebox{1\linewidth}{!} {
    \includegraphics{images/bar_step_position_acc_img.pdf}
  }
  \caption{The model's error-detection accuracy across diffrent error steps, truncated to 10.}
    \label{fig:bar_step_position_acc}
  \vspace{-4mm}
\end{figure}

==> sec/2_related.tex <==
\section{Related Work}
% \input{tables/statistics_ProJudgeBench}
% \input{tables/statistics}
\subsection{Multi-Modal Benchmarks}
With the fast development of recent MLLMs~\cite{ref:gemini_2_flash,ref:gpt4o,ref:qwen2.5-vl,ref:blip,ref:deepseekvl}, it becomes essential to evaluate their performance across a variety of tasks to understand their strengths and weaknesses, which is crucial for guiding future developments and enhancements~\cite{ref:mmmu,ref:mathvista,ref:eee-bench,ref:mmbench,ref:mmt-bench,masry2022chartqa,ref:seed-bench,ref:ok-bench,ref:docvqa,ref:wemath,qiao2024we,ref:math-vision,wang2025charxiv}. For example, MMMU~\cite{ref:mmmu} has been proposed to evaluate the scientific problem-solving abilities of MLLMs across a range of college-level subjects. MathVista~\cite{ref:mathvista} is widely used to assess the mathematical capabilities of MLLMs. While considerable progress has been achieved, these benchmarks often focus solely on evaluating final answers, overlooking crucial information of intermediate reasoning steps and potentially leading to unreliable results.
\subsection{MLLM-based Process Judges}
% As MLLMs regularly make mistakes when solving scientific problems~\cite{ref:mmmu,ref:mathverse}, evaluating the validity of their reasoning processes is critical for ensuring reliability and uncovering fine-grained model weaknesses. Since human evaluation is costly and time-consuming, prompting MLLMs as automated process judges has become a common practice.
% As MLLMs becomes increasingly capable in solving scientific problems, a central challenge is how to evaluate the multi-modal reasoning steps. While human evaluation has been the gold standard, it's costly and time-consuming for large-scale assessment. As an alternative, prompting MLLMs as automated process judges has become a scalable solution.
MLLM-based process judges have been widely used to automatically evaluate reasoning steps of multi-modal language models.
For example, 
MM-Math~\cite{ref:mm-math} incorporates MLLM-as-a-judge to automatically analyze solution steps, identifying and categorizing errors into specific error types. 
OlympicArena~\cite{ref:olympicarena} employs GPT-4V to conduct process-level evaluations, scoring the correctness of each reasoning step to ensure a rigorous assessment.
% MathVerse~\cite{ref:mathverse} employs GPT-4V to extract crucial reasoning steps, and then score each step with detailed error analysis, revealing the intermediate CoT reasoning quality by MLLMs. 
MathVerse~\cite{ref:mathverse} introduces a Chain-of-Thought (CoT) evaluation strategy, using GPT-4V to extract and assess key reasoning steps, providing fine-grained error analysis and nuanced scoring.
% that goes beyond binary correctness.
% MME-CoT~\cite{mme-cot} utilizes GPT-4o to assess the quality, robustness, and efficiency of Chain-of-Thought (CoT) reasoning  process in multimodal models.
MME-CoT~\cite{ref:mme-cot} extends this approach by evaluating CoT reasoning across multiple domains, while introducing metrics for reasoning quality, robustness, and efficiency.

Despite the widespread adoption, reliability of MLLMs-based judges themselves is rarely scrutinized. 
Besides, current evaluation predominantly relies on proprietary models, suffering from prohibitive costs and reproducibility instability. This necessitates the development of open-source process judges. To address these challenges, we introduce \textbf{ProJudgeBench}, a comprehensive benchmark for assessing MLLMs' capabilities as process judges, and \textbf{ProJudge-173k}, a large-scale instruction-tuning dataset designed to enhance open-source MLLMs' process evaluation abilities.
%In this paper, we introduce ProJudgeBench, a comprehensive benchmark, and ProJudge-173k, a large-scale instruction-tuning dataset, designed to evaluate and improve MLLMs' abilities in process evaluation.
%To address these challenges, we introduce ProJudgeBench, a comprehensive benchmark for assessing MLLMs-based process judges, and ProJudge-173k, a large-scale dataset designed to improve the process evaluation capabilities of open-source models.
% In this paper, we introduce ProJudgeBench and ProJudge-173k, laying the foundation for evaluating and improving capabilities of MLLMs-based process judges.


\subsection{Process Evaluation Benchmarks}
There exist several benchmarks related to assessing process evaluation abilities of LLMs. 
MR-GSM8K~\cite{ref:mr_gsm8k} introduces a meta-reasoning paradigm, requiring LLMs to transition from solving problems to evaluating the correctness of reasoning steps.
MathCheck-GSM~\cite{ref:mathcheck_gsm} presents a checklist-based framework, where LLMs are tasked with evaluating both final answers and intermediate reasoning steps.
CriticBench~\cite{ref:criticbench} assesses the ability of LLMs to critique and correct their reasoning across multiple domains.
ProcessBench~\cite{ref:processbench} measures the ability to identify erroneous steps in mathematical reasoning, particularly in competition-level problems.
PRMBench~\cite{ref:prmbench} synthesize erroneous steps based on PRM800k~\cite{ref:prm800k}, evaluating fine-grained error detection capabilities of PRMs across multiple dimensions.
% PRMBench evaluates the fine-grained error detection capabilities of PRMs across multiple dimensions, including simplicity, soundness, and sensitivity. 

Our ProJudgeBench is distinguished from prior benchmarks in three key aspects, as shown in Tabel~\ref{tab:comparison}. 
First, it covers four scientific discipline with multi-modal content and varying difficutly levels, reflecting the complexity of real-world reasoning tasks.
Second, test cases are curated from diverse model-generated solutions instead of synthetic data, capturing broad realistic reasoning behaviors and error patterns.
Third, each step is human-annotated for correctness, error type and explanation, enabling fine-grained evaluation of models' error-diagnosing capabilities.

==> sec/4_exp/0_main_res.tex <==
% \input{tables/main_res}
\input{images/radar}
\section{Experiments}
% \subsection{Experiment Setup}
% \textbf{Evaluation Models.} 
% To provide a comprehensive evaluation of various models on ProJudgeBench, we select a diverse set of both proprietary and open-source models. Proprietary models include GPT-4o~\cite{ref:gpt4o}, Gemini-2.0-flash-exp~\cite{ref:gemini_2_flash}, Gemini-2.0-thinking-exp~\cite{ref:gemini_2_flash_thinking}, and o1-mini~\cite{ref:o1}, while open-source models comprise InternVL2.5~\cite{ref:internvl2.5} (8B, 26B, 38B), MiniCPM-V-2\_6~\cite{ref:minicpm} (8B), and Qwen2.5-VL~\cite{ref:qwen2.5-vl} (3B, 7B, 72B). Additionally, we evaluate fine-tuned versions of InternVL2.5-8B, Qwen2.5-VL-3B, and Qwen2-VL-7B on ProJudge-173k.
To provide a comprehensive evaluation of various models on ProJudgeBench, we select a diverse set of both proprietary and open-source MLLMs, including GPT-4o~\cite{ref:gpt4o}, Gemini-2.0-flash-exp~\cite{ref:gemini_2_flash}, Gemini-2.0-thinking-exp~\cite{ref:gemini_2_flash_thinking}, o1-mini~\cite{ref:o1}, InternVL2.5~\cite{ref:internvl2.5} (8B, 26B, 38B), MiniCPM-V-2\_6~\cite{ref:minicpm} (8B), and Qwen2.5-VL~\cite{ref:qwen2.5-vl} (3B, 7B, 72B). Additionally, we evaluate fine-tuned versions of InternVL2.5-8B, Qwen2.5-VL-3B, and Qwen2-VL-7B.

% \noindent \textbf{Implementation Details.} 
% The input format and evaluation prompts for all models are kept consistent, with detailed descriptions provided in Appendix. For hyperparameters, we follow the settings in VLMEvalKit~\cite{ref:vlmevalkit}.
% We use accuracy as the primary evaluation metric, focusing on:
% (1) Step Correctness Accuracy: the accuracy of determining whether each step in a student's solution is correct.
% (2) Error Types Classification Accuracy: the accuracy of identifying specific error types, including Reasoning Errors (RE), Visual Interpretation Errors (VI), Numerical Calculation Errors (NC), Symbolic Calculation Errors (SC), Knowledge Errors (KE), Question Understanding Errors (QU), and No Solution Provided Errors (NS).
To ensure consistency, all models use the same input format and evaluation prompts, with hyperparameters following configurations in VLMEvalKit~\cite{ref:vlmevalkit}. We use accuracy as the primary evaluation metric, focusing on two aspects: (1) Step Correctness Accuracy, the accuracy of determining whether each step in a student's solution is correct; and (2) Error Types Classification Accuracy, the accuracy of identifying specific error types, including Reasoning Errors (RE), Visual Interpretation Errors (VI), Numerical Calculation Errors (NC), Symbolic Calculation Errors (SC), Knowledge Errors (KE), Question Understanding Errors (QU), and No Solution Provided Errors (NS).


\subsection{Main Results on ProJudgeBench}
The main results are presented in Table~\ref{tab:main}, from which we draw several key insights as follows:

\noindent \textbf{Model Scale Directly Impacts Process Evaluation Capabilities.}  
The performance of MLLMs demonstrates a clear trend: larger models exhibit significantly higher accuracies on both step correctness and error type classification.
Specifically, the InternVL2.5 series demonstrates a clear scaling effect, with the Step Correctness Accuracy increasing significantly from 25.58\% for InternVL2.5-8B to 66.72\% and 78.85\% for the 26B and 38B versions, respectively. Similarly, the Qwen2.5-VL models follow a comparable pattern, with the 72B version achieving the highest score (77.93\%), far surpassing the 3B (11.47\%) and 7B (34.65\%) versions.
In contrast, smaller models like MiniCPM-V-2\_6 exhibit weaker reasoning capabilities, with near-zero accuracy in several error categories.

\noindent \textbf{Proprietary Models Maintain a Performance Lead.}
% Proprietary models, particularly GPT-4o, consistently outperform the open-source models.
Proprietary models, particularly GPT-4o, demonstrate superior performance across the board. 
GPT-4o achieves the highest step correctness accuracy (85.10\%) and excels across multiple error categories, including RE (44.89\%), NC (40.90\%), and QU (30.10\%). The Gemini-2.0 series, while slightly behind GPT-4o, still outperforms most open-source models, with step correctness accuracy around 72.5\% and particularly excellent in identifying Visual Interpretation Errors. These results underscore the advanced reasoning and multimodal understanding capabilities of proprietary models. However, o1-mini, despite its strong performance in STEM-related tasks, falls short in this evaluation. We observed that it has difficulty adhering to the required output format specified in the evaluation prompt, leading to numerous outputs failing to extract the expected results.

\noindent \textbf{Fine-tuning Significantly Enhances Model Performance.}
Fine-tuning on ProJudge-173k yields substantial improvements across all models.
Open-source models like InternVL2.5-8B and Qwen2.5-VL-3B show dramatic gains, with step correctness accuracy increasing by 58.92\% and 70.45\%, respectively, bringing their performance on par with or even surpassing some proprietary models.
With sufficient fine-tuning, smaller models can approach the performance of much larger counterparts. For instance, Qwen2.5-VL-3B achieves 81.29\% accuracy after fine-tuning, nearly matching its much larger counterpart, Qwen2.5-VL-72B. These results highlight the transformative impact of domain-specific fine-tuning, enabling even smaller models to achieve competitive performance.

\noindent \textbf{Models Exhibit Unique Strengths Across Different Error Types.}
Different models exhibit distinct strengths in detecting specific error types. 
Although GPT-4o leads overall, open source models such as Qwen2.5-VL-72B and InternVL2.5-38B also excel in certain tasks. For example, Qwen2.5-VL-72B performs exceptionally well in identifying Reasoning Errors and Calculation Errors, while InternVL2.5-38B leads in detecting Knowledge Errors and Question Understanding Errors, highlighting the nuanced strengths of different model architectures.


==> sec/4_exp/1_further_analysis.tex <==
\input{images/heatmap}
\input{images/bar_making_and_indentifying_error}
\subsection{Further Analysis}

To gain deeper insights into the capabilities of MLLMs as process judges, we explore several key research questions: \textbf{RQ1}: How does model performance vary across different disciplines, difficulty levels, and modalities? \textbf{RQ2}: How do models perform as judges when assessing solutions from different student models? \textbf{RQ3}: What is the relationship between a model’s ability to detect errors and its tendency to make similar errors? Below, we discuss each research question in detail, providing a comprehensive understanding of models' performance characteristics and limitations in their role as process judges.

\subsubsection{RQ1: Performance Variation Across Domains and Modalities}
We analyze model performance across different domains (mathematics, physics, chemistry, biology), difficulty levels (primary school, middle school, high school, olympic), and modalities (pure text, single image, multi-images). The results, illustrated in Figure~\ref{fig:radar}, reveal several key insights into how MLLMs-based process judges perform in diverse scenarios.

\noindent \textbf{Most MLLMs exhibit varying performance across different domains, , with higher accuracy in biology and chemistry tasks compared to mathematics and physics.} 
For instance, InternVL2.5-38B achieves 82.08\% accuracy in biology but only 73.14\% in mathematics, while Qwen2.5-VL-72B achieves 84.13\% in biology but 77.08\% in physics.
This discrepancy can be attributed to the nature of the tasks: biology and chemistry problems often rely on factual knowledge and rule-based reasoning, such as identifying biological classifications or balancing chemical equations, which align well with models’ ability to parse and validate logical sequences. These tasks involve clear, well-defined rules and less abstract reasoning, making them easier for models to evaluate.
In contrast, mathematics and physics demand complex logical reasoning, multi-step derivations, and the ability to handle abstract concepts. For example, solving a physics problem may involve applying multiple formulas and interpreting real-world scenarios, posing a greater challenge for models. Similarly, mathematical tasks, despite their structured nature, require precise logical validation, leading to misjudgments when models fail to grasp subtle errors in reasoning.
The performance gap highlights the need for models to develop more robust reasoning mechanisms to handle the complexity and abstraction inherent in physics and mathematics.

\noindent \textbf{As task difficulty increases, the model's accuracy in step evaluation consistently declines.} 
For instance, Gemini-2.0 achieves 80.2\% accuracy in high school tasks but drops to 56.2\% in OlympiadBench tasks, while InternVL2.5-8B shows a more pronounced decline, from 34.1\% in primary school to 22.3\% in OlympicArena.
This trend highlights the challenges models face when dealing with complex, multi-step reasoning tasks, which require not only advanced domain knowledge but also the ability to synthesize information and apply it in novel ways. Current models often struggle with these requirements, leading to lower accuracy in step evaluation.
Interestingly, primary school tasks do not always show the highest accuracy, despite their relative simplicity. 
This counterintuitive result can be attributed to the diverse and context-dependent nature of primary school tasks, which may involve unconventional reasoning steps or less structured problem-solving approaches. While these tasks are simpler in terms of content, their variability and lack of standardized reasoning patterns can pose challenges for models trained on more formal and structured datasets.

\noindent \textbf{While proprietary models like GPT-4o achieve relatively balanced performance across modalities, open-source models tend to excel in pure text tasks but face significant challenges in tasks involving single or multiple images.} 
For example, gpt-4o maintains 84.5\% accuracy in single-image tasks and 83.9\% in multi-image tasks, while MiniCPM-V-2\_6 drops from 21.5\% in pure text tasks to 11.6\% in multi-image tasks. 
Pure text tasks rely solely on textual information, which aligns well with the core capabilities of language models, enabling more accurate step evaluation. In contrast, tasks involving images require models to process and interpret visual elements, such as diagrams, charts, or graphs, and integrate them with textual reasoning, leading to increased challenges in maintaining accuracy.
This disparity highlights the limitations of current open-source models in integrating and interpreting visual information alongside textual reasoning, which remains a significant bottleneck in multimodal process evaluation.
Notably, single-image tasks tend to outperform multi-image tasks across most models, indicating that combining information from multiple images adds complexity and reduces evaluation accuracy.



\subsubsection{RQ2: Model-as-Judge Performance Across Different Student Models}
Figure~\ref{fig:heatmap} illustrates the performance of different models acting as process judges when evaluating solutions generated by other models (student models). Each position (x, y) in the heatmap represents the accuracy of model x as a judge in assessing the correctness of steps generated by model y. From the figure, we observe several key patterns that provide insights into the capabilities and limitations of MLLMs in cross-model process evaluation.

First, we find that models InternVL series models demonstrate higher accuracy when evaluating themselves or models from the same series.
This can be attributed to the shared architectures, training data, and reasoning styles within the same series, enabling them to better understand and assess the reasoning processes and error patterns of their counterparts.
This suggests a potential approach: smaller could submit intermediate steps to larger models for verification, where larger models could provide high-quality error feedback to help improve their reasoning capabilities.
Besides, we observe that larger models tend to achieve higher accuracy when evaluating smaller models, whereas smaller models struggle to assess larger ones effectively. For example, GPT-4o reaches 84.31\% accuracy when evaluating MiniCPM-V-2\_6, while MiniCPM-V-2\_6 achieves only 15.69\% accuracy when evaluating GPT-4o. This discrepancy indicates the superior reasoning abilities and broader training data of larger models, which enable them to better understand and assess the reasoning processes of smaller models. In contrast, smaller models, constrained by their limited capacity, often struggle to accurately evaluate the more complex reasoning steps of larger models.


\subsubsection{RQ3: Correlation Between Error Detection and Error Generation}
Given that models exhibit varying capabilities in detecting different types of errors, we aim to explore the relationship between error types and the models' ability to identify them. To this end, we analyze the performance of two MLLM-based process judges, InternVL2.5-38B and Qwen2.5-VL-72B, across five error types, examining both the frequency of generating these errors and the accuracy of detecting them.
The results are shown in Figure~\ref{fig:bar_making_and_identifying_error}, from which we draw the following key observations:

First, for visual interpretation errors, both models exhibit high error generation rates and low detection accuracy. This suggests that, despite their multimodal architecture, the models struggles with interpreting and reasoning about visual information, revealing limitations in their ability to process and align multimodal data.
Second, regarding calculation errors, both models have a relatively high error generation frequency and also notable detection accuracy. This indicates that while models are prone to calculation errors, they possess a reasonable ability to identify such errors. This finding highlights the potential for reducing such errors by introducing self-checking mechanisms.
For knowledge errors, both models show relatively low error generation frequency and detection accuracy. This suggests that, while pre-trained knowledge ensures general stability, models lack expertise in domain-specific understanding. As a result, they are prone to making errors when dealing with domain knowledge and struggle to detect these errors. Targeted training on the relevant knowledge points could help strengthen their performance in these areas.
For question understanding and no solution provided errors, both models show low frequencies of errors generation. InternVL2.5-38B achieves higher detection accuracy for question understanding errors, likely due to the strong language comprehension capabilities of its base language model.

==> sec/4_exp/2_ablation.tex <==
\subsection{Ablation Study}
\input{tables/ablation}
In this section, we conduct a comprehensive ablation study to evaluate our Dual-Phase (DP) fine-tuning strategy and training data composition effects. As shown in Table~\ref{tab:ablation}, we explore several configurations: standard fine-tuning (+FT) versus DP-enhanced training (+DP), and training on K12 only, OlympiadBench only, or the combined set. Beyond overall step correctness accuracy, we delve into three test subsets—K12, OlymiadBench, and the unseen OlymicArena—to assess both in-domain performance and generalization capabilities. All models are fine-tuned using LoRA for one epoch (see Appendix for details).

The results demonstrate that DP consistently improves performance across all models, with particularly notable gains in generalization to unseen problem types. 
On the challenging OlymicArena test set, which contains entirely novel competition-level questions, DP-enhanced models achieve significant performance boosts—InternVL2.5-8B improves by 3.36\%, while QwenVL2.5-7B gains 4.79\%. This suggests that the explicit problem-solving phase in DP not only deepens the model's understanding of scientific reasoning, but also enhances its robustness to evaluate unfamiliar solution strategies.

Training on the combined dataset yields the best overall performance, as it benefits from both the broad coverage of foundational knowledge in K12 and the advanced reasoning challenges in OlympiadBench. Interestingly, models trained exclusively on K12 data outperform those trained only on OlympiadBench, despite the latter's higher problem difficulty. 
This can be attributed to the larger size and greater diversity of the K12 training set, which covers four disciplines (mathematics, physics, chemistry, and biology) and multiple difficulty levels. In contrast, the OlympiadBench training set, while more challenging, is limited to mathematics and physics, resulting in a narrower scope of learning.
These findings underscore the importance of balancing data difficulty with diversity to achieve robust and generalizable performance.


==> tables/statistics_ProJudgeBench.tex <==
\begin{table*}[tp]
  \centering
  \resizebox{0.78\textwidth}{!}{
  \begin{tabular}{lccccccccc}
    \toprule[0.8pt]
    \multirow{2}{*}{}
    & \multirow{2}{*}{\textbf{Overall}}  
    & \multicolumn{2}{c}{\textbf{Math}}  
    & \multicolumn{2}{c}{\textbf{Physics}}
    & \multicolumn{2}{c}{\textbf{Chemistry}}
    & \multicolumn{2}{c}{\textbf{Biology}}\\
    \cmidrule(){3-4} \cmidrule(){5-6} \cmidrule(){7-8} \cmidrule(){9-10} 
    && \textbf{K12} & \textbf{Comp} & \textbf{K12} & \textbf{Comp} & \textbf{K12} & \textbf{Comp} &\textbf{K12} & \textbf{Comp}   \\
     \midrule
    
    \# Samples & 2400 & 450 & 150 & 300 & 300 & 300 & 300 & 300 & 300 \\
    Avg. Steps & 20.8 & 23.7 & 21.3 & 21.5 & 26.0 & 20.0 & 19.9 & 15.2 & 18.0 \\
    Max. Steps & 470 & 470 & 215 & 199 & 353 & 209 & 197 & 78 & 150 \\
    \% Error Steps & 21.6 & 23.0 & 19.7 & 21.2 & 23.1 & 18.9 & 24.4 & 15.7 & 23.4 \\
    Avg. Error Steps & 6.6 & 8.1 & 7.0 & 7.0 & 8.4 & 5.7 & 6.2 & 4.2 & 5.7 \\
    % Max. Error Steps & 226 & 226 & 32 & 64 & 57 & 41 & 74 & 17 & 49 \\
    Max. Error Types & 5 & 4 & 4 & 4 & 4 & 4 & 5 & 3 & 4 \\
    
    \bottomrule[0.8pt]
    
  \end{tabular}
  }
  \caption{Statistics of ProJudgeBench. K12 and Comp represent normal and competition-level problems, respectively.}
  \label{tab:statistics_ProJudgeBench}
  \vspace{-4mm}
\end{table*}


% \begin{table}[tp]
%   \centering
%   \resizebox{0.5\textwidth}{!}{
%   \begin{tabular}{lccccccccc}
%     \toprule[0.8pt]
%     \multirow{2}{*}{}
%     & \multirow{2}{*}{\textbf{Overall}}  
%     & \multicolumn{4}{c}{\textbf{Disciplines}}  
%     & \multicolumn{2}{c}{\textbf{Difficulty}} \\
%     \cmidrule(){3-6} \cmidrule(){7-8}
%     && \textbf{Math} & \textbf{Phy.} & \textbf{Chem.} & \textbf{Bio.} & \textbf{K12} & \textbf{Comp} \\
%      \midrule
    
%     \# Samples & 2400 & 450 & 150 & 300 & 300 & 300 \\
%     Avg. Steps & 20.8 & 23.7 & 21.3 & 21.5 & 26.0 & 20.0 \\
%     Max. Steps & 470 & 470 & 215 & 199 & 353 & 209 \\
%     \% Err Steps & 21.6 & 23.0 & 19.7 & 21.2 & 23.1 & 18.9 \\
%     Avg. Err Steps & 6.6 & 8.1 & 7.0 & 7.0 & 8.4 & 5.7 \\
%     % Max. Error Steps & 226 & 226 & 32 & 64 & 57 & 41 & 74 & 17 & 49 \\
%     Max. Err Types & 5 & 4 & 4 & 4 & 4 & 4 \\
    
%     \bottomrule[0.8pt]
    
%   \end{tabular}
%   }
%   \caption{Statistics of ProJudgeBench. K12 and Comp represent normal and competition-level problems, respectively.}
%   \label{tab:statistics_ProJudgeBench}
%   \vspace{-4mm}
% \end{table}

